Structured risk model

Income and risk coexist, yet investors are often so focused on chasing high returns that they overlook the potential risks that can lead to high losses. Therefore, risk forecasting and risk control is the cornerstone of investment. To address the challenge, we construct a multi-factor risk model on the basis of the classical multi-factor modeling framework. For the common factors, inspired by Barra Model's factor classification. we adjust the outliers and missing values of factor exposure data, normalize and finally orthogonalize them, before computing factor returns and making further analysis. Factor return covariance matrix and idiosyncratic return variance matrix are essential tools to express stock returns in the multi-factor risk model. Firstly, we calculate the factor return covariance matrix with EWMA. To tackle the time-series autocorrelation of factor returns, we apply Newey-West adjustment. Then we estimate the idiosyncratic return variance matrix in a similar way and make Newey-West adjustment again to solve the time-series autocorrelation problem. Since the return of a single share is sensitive to missing values and outliers, we introduce structural adjustment to improve the matrix.Eventually, we obtain the return covariance matrix among stocks and compute the risk of investment portfolio based on it. Furthermore, we search for optimal portfolio with respect to minimizing risk or maximizing risk-adjusted return with our model. They provide good Sharpe ratio and information ratio for considering both absolute risk and active risk. Hence, the multi-factor risk model is efficient.

==> title.tex <==
\begin{titlepage}
   \begin{center}
       \vspace*{1cm}
       \includegraphics[width=0.8\textwidth]{./fos-logo.png}\\
       
	\huge
	
	
       \textbf{QF5206 Project}

	\large
       \vspace{0.5cm}

       \vspace{1.5cm}

       \textbf{}\\
	 \textbf{}
	 
       \vfill
            
            
       \vspace{0.8cm}
     
	National University of Singapore\\
	Wu Yiqiao (A0251201A)\\
	Jing Zhiqi (A0253630M)\\
	Huang Qianying (A0253869L)\\
	Zhu Zhiyi (A0251088A)\\
	Ma Yufei (A0177864L)\\
       Song Xinyuan (A0251554H)\\
~\\
~\\

\small

   \end{center}
\end{titlepage}
